DepressionNet: A Novel Summarization Boosted Deep Framework for Depression Detection on Social Media

Twitter is currently a popular online social media platform which allows users to share their user-generated content. This publicly-generated user data is also crucial to healthcare technologies because the discovered patterns would hugely benefit them in several ways. One of the applications is in automatically discovering mental health problems, e.g., depression. Previous studies to automatically detect a depressed user on online social media have largely relied upon the user behaviour and their linguistic patterns including user's social interactions. The downside is that these models are trained on several irrelevant content which might not be crucial towards detecting a depressed user. Besides, these content have a negative impact on the overall efficiency and effectiveness of the model. To overcome the shortcomings in the existing automatic depression detection methods, we propose a novel computational framework for automatic depression detection that initially selects relevant content through a hybrid extractive and abstractive summarization strategy on the sequence of all user tweets leading to a more fine-grained and relevant content. The content then goes to our novel deep learning framework comprising of a unified learning machinery comprising of Convolutional Neural Network (CNN) coupled with attention-enhanced Gated Recurrent Units (GRU) models leading to better empirical performance than existing strong baselines.

==> figures/TNSE_BertBart.tex <==



\begin{figure*}[!htb]
\centering
  \begin{subfigure}[b]{.23\linewidth}
    \centering
 \includegraphics[width=.99\textwidth]{images/TSNE/Bert-Bart_280.png}
    \caption{Optimization iterations = 280}\label{fig:1a}
  \end{subfigure}%   
  \begin{subfigure}[b]{.23\linewidth}
    \centering
   
  \includegraphics[width=.99\textwidth]{images/TSNE/Bert-Bart_290.png}
    \caption{Optimization iterations = 290}\label{fig:1b} 
  \end{subfigure}%  
 \begin{subfigure}[b]{.23\linewidth}
    \centering
    \includegraphics[width=.99\textwidth]{images/TSNE/Bert-Bart_300.png}
    \caption{Optimization iterations = 300}\label{fig:1c}
 \end{subfigure}%  
   \begin{subfigure}[b]{.23\linewidth}
     \centering
   \includegraphics[width=.99\textwidth]{images/TSNE/Bert-Bart_310.png}
    \caption{Optimization iterations = 310}\label{fig:1d}
   \end{subfigure}%   
       \vspace{0.5cm}

   \caption{t-SNE visualization of Bert-Bart Summarization, where (1) represent depressed users posts and (0) represent non-depressed users posts}\label{fig:Bert-Bart}
\end{figure*}

==> figures/TSNE_BertDistilBart.tex <==



\begin{figure*}[htb]
\centering
  \begin{subfigure}[b]{.24\linewidth}
    \centering
    \includegraphics[width=.99\textwidth]{images/TSNE/Bert-DistilBart_280.png}
    \caption{Optimization iterations = 280}\label{fig:1a}
  \end{subfigure}%   
  \begin{subfigure}[b]{.24\linewidth}
    \centering
    \includegraphics[width=.99\textwidth]{images/TSNE/Bert-DistilBart_290.png}
    \caption{Optimization iterations = 290}\label{fig:1b}
  \end{subfigure}%  
  \begin{subfigure}[b]{.24\linewidth}
    \centering
    \includegraphics[width=.99\textwidth]{images/TSNE/Bert-DistilBart_300.png}
    \caption{Optimization iterations = 300}\label{fig:1c}
  \end{subfigure}%  
  \begin{subfigure}[b]{.24\linewidth}
    \centering
    \includegraphics[width=.99\textwidth]{images/TSNE/Bert-DistilBart_310.png}
    \caption{Optimization iterations = 310}\label{fig:1d}
  \end{subfigure}%   
      \vspace{0.5cm}

  \caption{t-SNE visualization of Bert-DistilBart Summarization, where (1) represent depressed users posts and (0) represent non-depressed users posts}\label{fig:Bert-DistilBart}
  \vspace{1cm}
\end{figure*}

==> figures/bart_model.tex <==
\begin{figure}
  \centering
  \includegraphics[scale=0.2]{images/BART1_.png}
  \caption{BART: Denoising Sequence-to-Sequence }
\label{fig:bart}
\end{figure}

==> figures/bert_bart_cluster.tex <==



\begin{figure*}[htb]
\centering
  \begin{subfigure}[b]{.30\linewidth}
    \centering
    \includegraphics[width=.99\textwidth]{images/TSNE/count_Bertbart.png}
    \caption{Using count of words}\label{fig:1a}
  \end{subfigure}%   
  \begin{subfigure}[b]{.30\linewidth}
    \centering
    \includegraphics[width=.99\textwidth]{images/TSNE/tf_Bertbart.png}
    \caption{Using TF}\label{fig:1b}
  \end{subfigure}%  
  \begin{subfigure}[b]{.30\linewidth}
    \centering
    \includegraphics[width=.99\textwidth]{images/TSNE/tfidf_Bertbart.png}
    \caption{Using TF-IDF}\label{fig:1c}
  \end{subfigure}%  
      \vspace{0.5cm}

   \caption{t-SNE visualization of Bert-Bart Summarization, with  }\label{fig:Bert-Bart}
\end{figure*}

==> figures/bert_distilbart_cluster.tex <==



\begin{figure*}[htb]
\centering
  \begin{subfigure}[b]{.30\linewidth}
    \centering
    \includegraphics[width=.99\textwidth]{images/TSNE/count_BertDistilbart.png}
    \caption{Using count of words}\label{fig:1a}
  \end{subfigure}%   
  \begin{subfigure}[b]{.30\linewidth}
    \centering
    \includegraphics[width=.99\textwidth]{images/TSNE/tf_BertDistilbart.png}
    \caption{Using TF}\label{fig:1b}
  \end{subfigure}%  
  \begin{subfigure}[b]{.30\linewidth}
    \centering
    \includegraphics[width=.99\textwidth]{images/TSNE/tfidf_BertDistilbart.png}
    \caption{Using TF-IDF}\label{fig:1c}
  \end{subfigure}%  
      \vspace{0.5cm}

   \caption{t-SNE visualization of Bert-DistilBart Summarization, with  }\label{fig:Bert-Bart}
\end{figure*}

==> figures/cloud_non_depressed.tex <==
\begin{figure}%
    \centering
    \subfloat[\centering Before ]{{\includegraphics[width=4.3cm]{images/non_depressed_pre.png} }}%
    \subfloat[\centering After ]{{\includegraphics[width=4.3cm]{images/non_depressed_post.png} }}%
    
    
     \vspace{0.3cm}
    \caption{A word cloud for a non-depressed user posts before and after extractive summarization}%
    \label{fig:cloud_dep}%
\end{figure}

==> figures/results_figures.tex <==
\begin{figure*}%
    \centering
    \subfloat[\centering - Effectiveness of summarization sequence with modality ]{{\includegraphics[scale=0.2530]{images/Seq_with_modalties.png} }}%
   % \vspace{0.3cm}
    \subfloat[\centering - Effectiveness of our model with modality ]{{\includegraphics[scale=0.25]{images/model_modalities.png} }}%
     %\vspace{0.3cm}
   \caption{Experimental results: (a) Comparing the performance of our model by concatenating sequences with different modalities. (b) Showing the performance of our model by omitting different modalities.}
   \label{fig: Model_results_performance}%
\end{figure*}








==> figures/results_figures_.tex <==
\begin{figure*}%
\small
    \centering
    \subfloat[\centering - Effectiveness of summarization sequence with modality ]{{\includegraphics[scale=0.4]{images/Seq_with_modalties.png} }}%
    \subfloat[\centering - Effectiveness of our model with modality ]{{\includegraphics[scale=0.4]{images/model_modalities.png} }}%
     \vspace{0.3cm}
     %2530
            \subfloat[\centering - Statistics about depression symptoms ]{{\includegraphics[scale=0.35]{images/symptoms.png} }}
         \subfloat[\centering -BART  ]{{\includegraphics[scale=.30]{images/TSNE/tf_Bertbart.png} }}
    \subfloat[\centering - DistilBART  ]{{\includegraphics[scale=0.30]{images/TSNE/tf_BertDistilbart.png} }}
\vspace{0.12cm}
   \caption{Experimental results: (a) Comparing the performance of our model by concatenating sequences with different modalities. (b) Showing the performance of our model by omitting different modalities. (c) The most common symptoms among depressed users. (d) and (e) T-SNE visualization of Bart and DistilBart Summarization, where 1 represent depressed users posts and 0 represent non-depressed users posts}
   \label{fig: Model_results_performance}%
\end{figure*}








==> figures/results_figures_2.tex <==
\begin{figure*}%
    \centering
    \subfloat[\centering - Statistics about depression symptoms ]{{\includegraphics[scale=0.23]{images/symptoms.png} }}
    \vspace{0.3cm} 
    \subfloat[\centering - Visualization of Bart Summarization ]{{\includegraphics[width=3cm]{images/TSNE/tf_Bertbart.png} }}
    \subfloat[\centering - Visualization of DistilBart Summarization ]{{\includegraphics[width=3cm]{images/TSNE/tf_BertDistilbart.png} }}
     \vspace{0.3cm}
   \caption{(a) The most common symptoms among depressed users. (b) and (c) T-SNE visualization of Bart and DistilBart Summarization, where 1 represent depressed users posts and 0 represent non-depressed users posts.}\label{fig: symptoms_tsne}%
\end{figure*}










==> images/mainflow.tex <==
% \section{Diagrammatic view of Multisketch operations}\label{app:mainflow}  

% A user registers with a user id $\u$ and a vector of biometric templates
% $\mvec=\mvecss{\mlen}$. Multisketch uses two databases $\dbid$ and $\dbmsg$\@,
% where $\dbid$ contains user id $\u$ and the corresponding helper data
% $\sketchval$, and $\dbmsg$ contains the random permutation of the templates
% registered so far. Highlighted are the entries corresponding to a user $\u_4$
% with templates $\mvec_4=\mvec_{41}\ldots\mvec_{4\mlen}$.% and helper
%     % data $\sketchval_4$.
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
    >=stealth,
    node distance=2cm,
    database/.style={
      cylinder,
      cylinder uses custom fill,
      cylinder body fill=black!25!white,
      cylinder end fill=black!25!white,
      shape border rotate=90,
      aspect=0.25,
      minimum width=2em,
      minimum height=2em,
      draw
    },
    func/.style={
      rectangle,
      fill=red!25!white,
      minimum width=1cm,
      minimum height=1em,
      draw
    },
    cell/.style={
      rectangle,
      draw=black!50!white
    }
    ]
    \node (user) at (0, 0) {User};
    \node[func, right of=user, right=-1.1em, above=3em] (msketch) {$\MS$}; 
    \draw[below of=msketch, dashed, anchor=west] (.85,0.55) rectangle (5.9,-1.2); 
    \node[func, below of=msketch, anchor=east, below=1.95cm,fill=red!10!white,dashed] (mrecover) {$\MRec$};
    % \node[database, right of=user, anchor=south, above=1em, right=2cm] (db1) {$\dbid$};
    \matrix (db1) [right of=user, anchor=south, below=2pt, right=-0.1cm, 
    matrix of math nodes,
    column sep = -\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}}, 
    column 2/.style={nodes={cell}}, 
    anchor=west] {
      \u_1 & \sketchval_1\\
      \u_2 & \sketchval_2\\
      \u_3 & \sketchval_3\\
      |[draw,fill=blue!20]|\u_4 & |[draw,fill=blue!20]|\sketchval_4\\
    };
    \node[left of=db1, anchor=east,right=1.1cm] {$\dbid$};
    \matrix (db2) [right of=db1, left=25pt, matrix of math nodes,
    column sep = 2\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}},
    column 2/.style={nodes={cell}}, 
    column 3/.style={nodes={cell}}, 
    column 4/.style={nodes={cell}}, 
    column 5/.style={nodes={cell}}, 
    anchor=west] {
      \mvec_{21} &\mvec_{12} & |[draw,fill=blue!20]|\mvec_{43} &  & \mvec_{3\mlen} \\
      |[draw,fill=blue!20]|\mvec_{41} &\mvec_{32} & \mvec_{33} & |[draw=white]|\ldots & \mvec_{2\mlen} \\
      \mvec_{11} &|[draw,fill=blue!20]|\mvec_{42} & \mvec_{23} &  & \mvec_{1\mlen} \\
      \mvec_{31} &\mvec_{22} & \mvec_{13} & & |[draw,fill=blue!20]|\mvec_{4\mlen} \\
    };
    \node[left of=db2, left=-4pt] {$\dbmsg$};

    % \node[database,right of=db1] (db2) {$\dbmsg$};
    \node[func,below of=db1,anchor=north,above=8pt,left=8pt] (gu) {GetUser};
    \node[func,right of=gu,anchor=east,right=-5pt] (fm) {FindMatches};
    \node[func,below of=db1,anchor=east,below=2em,right=-3pt] (recover) {Recover};

    \draw[->,blue!50,thick] (user.north) |- node[black,near end,above]{$u, \mvec$} node[black,near end,below,font=\small]{register} 
    (msketch.west);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$u, \sketchval$} (db1);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$\mvec$} (db2);

    \draw[->,blue!50,thick] (user.south) |- ++(1,-0.9) node[black,near end,above]{$u, \mvectilde$} node[black,near end,below,font=\small]{login}   -| node[black,left,near end]{$u$}
    (gu.north);
    \draw[->,blue!50,thick] (user.south) |- ++(0,-0.9)  -- ++(3.1,0) |- node[black,near end, above]{$\mvectilde$}
    (fm.west);
    \draw[->,blue!50,thick] (db1.south) |- node[black,near end,above]{} (gu.east);
    \draw[->,blue!50,thick] (db2.south) |- node[black,near end,above]{} (fm.east);
    \draw[->,blue!50,thick] (gu.south) |- node[black,near end,above]{$\sketchval$} (recover.west);
    \draw[->,blue!50,thick] (fm.south) |- node[black,near end,above]{$\mvec'$} (recover.east);    
    \draw[->,blue!50,line width=2pt] (recover.south) -- node[black,near end,right]{$\mvec$ or $\bot$} ++(0, -0.65);
  \end{tikzpicture}
  % \rcnote{Rough sketch of the flow of the \biosketch.} 
  \caption{Diagram of multisketch as a part of an authentication service. 
  }
  \label{fig:mainflow}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tables/table_result_2.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}
  \centering
 % \vspace{0.3cm}
  
  \caption{Comparison of different models with our model for detection depression using summarization sequence and user behaviours.}
  \scalebox{0.7}
  {
    \begin{tabular}{p{12.0em}llll}
    \toprule
    \toprule
    \textbf{Model} & \multicolumn{1}{p{2.5em}}{\textbf{Prec.}} & \multicolumn{1}{p{2.5em}}{\textbf{Rec.}} & \multicolumn{1}{p{2.5em}}{\textbf{F1}} & \multicolumn{1}{p{2.5em}}{\textbf{Acc.}} \\
    \midrule
    BiGRU (Att) + BiGRU & 0.896 & 0.885 & 0.880 & 0.881 \\
    CNN + BiGRU & 0.880 & 0.866 & 0.860 & 0.861 \\
    CNN-BiGRU (Att) + BiGRU & 0.900 & 0.892 & 0.887 & 0.887 \\
    BiGRU (Att) + Stacked\_BiGRU & 0.906 & 0.901 & 0.898 & 0.898 \\
    CNN (Att) + Stacked\_BiGRU & 0.874 & 0.870 & 0.867 & 0.867 \\
    DepressionNet & \textbf{0.909} & \textbf{0.904} & \textbf{0.901} & \textbf{0.901} \\
    \bottomrule
    \bottomrule
    \end{tabular}%
    }
      \label{tab:seq_beha}%
      \vspace{-0.3cm}
\end{table}%


